Are Your Models Still Fair? Fairness Attacks on Graph Neural Networks via Node Injections

Despite the remarkable capabilities demonstrated by Graph Neural Networks (GNNs) in graph-related tasks, recent research has revealed the fairness vulnerabilities in GNNs when facing malicious adversarial attacks. However, all existing fairness attacks require manipulating the connectivity between existing nodes, which may be prohibited in reality. To this end, we introduce a Node Injection-based Fairness Attack (NIFA), exploring the vulnerabilities of GNN fairness in such a more realistic setting. In detail, NIFA first designs two insightful principles for node injection operations, namely the uncertainty-maximization principle and homophily-increase principle, and then optimizes injected nodes' feature matrix to further ensure the effectiveness of fairness attacks. Comprehensive experiments on three real-world datasets consistently demonstrate that NIFA can significantly undermine the fairness of mainstream GNNs, even including fairness-aware GNNs, by injecting merely 1% of nodes. We sincerely hope that our work can stimulate increasing attention from researchers on the vulnerability of GNN fairness, and encourage the development of corresponding defense mechanisms. Our code and data are released at: https://github.com/CGCL-codes/NIFA.

==> theoretical.tex <==
For the conciseness of formulation, we assume each injected node in $\mathcal{V}_I$ has degree $d$, i.e. connects with $d$ real nodes in the original graphs. Then, following prior work \cite{10.1145/3485447.3512201}, we utilize the node-level homophily-ratio $\mathcal{H}_u$ to represent the ratio of that connect the node $u$ and
another node $v$ with the same sensitive attribute, i.e. $\mathcal{H}_u=\frac{\sum_{\langle u, v \rangle \in \mathcal{N}_u}\mathbb{I}(s_u = s_v)}{|\mathcal{N}_u|}$, where $\mathcal{N}_u$ denotes the neighbors of node $u$. Then we can have:

\begin{lemma}
    Contrastive node injection will lead to the increase of node-level homophily-ratio $\mathcal{H}$.
\end{lemma}

Due to space limitation, the proof for Lemma~\ref{homo} is provided in the Appendix.

\begin{proof}
    Given a target node $u$ with $k$ neighbors with the same sensitive attribute, since all injected nodes in contrastive node injection belong to the same sensitive attribute as target node $u$, then the node-level homophily-ratio after node injection $\mathcal{H}^{\prime}_u$ is:
    \begin{equation}
    \mathcal{H}^{\prime}_u=\frac{k+|\mathcal{V}_I|*d}{|\mathcal{N}_u|+|\mathcal{V}_I|*d} \geq \frac{k}{|\mathcal{N}_u|}=\mathcal{H}_u
    \end{equation}
\end{proof}
